POSIX: A Prompt Sensitivity Index For Large Language Models

Despite their remarkable capabilities, Large Language Models (LLMs) are found to be surprisingly sensitive to minor variations in prompts, often generating significantly divergent outputs in response to minor variations in the prompts, such as spelling errors, alteration of wording or the prompt template. However, while assessing the quality of an LLM, the focus often tends to be solely on its performance on downstream tasks, while very little to no attention is paid to prompt sensitivity. To fill this gap, we propose POSIX - a novel PrOmpt Sensitivity IndeX as a reliable measure of prompt sensitivity, thereby offering a more comprehensive evaluation of LLM performance. The key idea behind POSIX is to capture the relative change in loglikelihood of a given response upon replacing the corresponding prompt with a different intent-preserving prompt. We provide thorough empirical evidence demonstrating the efficacy of POSIX in capturing prompt sensitivity and subsequently use it to measure and thereby compare prompt sensitivity of various open-source LLMs. We find that merely increasing the parameter count or instruction tuning does not necessarily reduce prompt sensitivity whereas adding some few-shot exemplars, even just one, almost always leads to significant decrease in prompt sensitivity. We also find that alterations to prompt template lead to the highest sensitivity in the case of MCQ type tasks, whereas paraphrasing results in the highest sensitivity in open-ended generation tasks. The code for reproducing our results is open-sourced at https://github.com/kowndinya-renduchintala/POSIX.

==> files/related_work.tex <==
\section{Related Works}

\noindent \textbf{Sensitivity of LLMs to prompt variations.} Several recent works \cite{sclar2023quantifying, voronov2024mind, mizrahi2024state, arora2022ask} have studied the issue of sensitivity of LLMs to minor alterations in the input prompt, with few of them calling for extending the evaluation benchmarks to include multiple versions for each prompt to account for the divergence in behavior of the models to prompt variations. Majority of these works \cite{sclar2023quantifying, mizrahi2024state, voronov2024mind} have examined the effect of change in only prompt template on model predictions. \citet{gu-etal-2023-robustness} looked into the robustness of LLMs' to various perturbations of instruction in prompts. 

However, these studies employ different metrics to quantify sensitivity, which include: {\em performance spread}, i.e., the difference between the maximum and minimum performance on a dataset with various prompt formats~\citep{sclar2023quantifying}, {\em variation ratio}, which is based on the frequency of the mode of outputs~\citep{lu2023prompts}, etc.


\noindent \textbf{Prompt engineering.} Due to such extensive variation in the performance of LLMs on slight modifications in input prompt, it is crucial to 
